DecompDiff: Diffusion Models with Decomposed Priors for Structure-Based Drug Design

Designing 3D ligands within a target binding site is a fundamental task in drug discovery. Existing structured-based drug design methods treat all ligand atoms equally, which ignores different roles of atoms in the ligand for drug design and can be less efficient for exploring the large drug-like molecule space. In this paper, inspired by the convention in pharmaceutical practice, we decompose the ligand molecule into two parts, namely arms and scaffold, and propose a new diffusion model, DecompDiff, with decomposed priors over arms and scaffold. In order to facilitate the decomposed generation and improve the properties of the generated molecules, we incorporate both bond diffusion in the model and additional validity guidance in the sampling phase. Extensive experiments on CrossDocked2020 show that our approach achieves state-of-the-art performance in generating high-affinity molecules while maintaining proper molecular properties and conformational stability, with up to -8.39 Avg. Vina Dock score and 24.5 Success Rate. The code is provided at https://github.com/bytedance/DecompDiff

==> sections/10-intro-backup.tex <==
\section{Introduction}
\label{sec:intro}

Modern deep learning is revolutionizing many subfields in drug discovery, among which 
structure-based drug design (SBDD) \citep{anderson2003process} is an important yet challenging one. 
Aiming at generating 3D ligand molecules conditioned on a target binding site, SBDD requires models to generate drug-like molecules with stable 3D structures and high binding affinities to the target. 
Recently, powerful deep generative models \todoq{add references here} have been proposed to achieve this goal.
They often treat the ligand molecule as a whole and learn the overall correspondence between the target binding site and the ligand. 
However, atoms within the same ligand can be designed for different functions. Therefore, treating all ligand atoms equally may not be the best way for SBDD, especially considering the tremendous drug-like space \citep{virshup2013stochastic} to explore and the limited amount of high quality target-ligand complexes \citep{berman2000protein} for training.
This motivates us to study how to properly incorporate function-related prior knowledge into SBDD methods.
% TODO: I cannot select one representative publication for molecule property prediction.


Decomposing ligands into smaller functional regions is a common practice in conventional drug design. However, it is underexplored in deep learning-based SBDD methods such as deep generative models. 
As shown in Figure~\ref{fig:decomp}, ligands can be decomposed into scaffold and arms. 
The arms are responsible for interacting with the target to achieve high binding affinity, while the scaffold is responsible for positioning the arms into the desired binding regions. 
In lead optimization, a scaffold is identified first, and then a series of analogs are developed by altering the arms for further activity optimization \citep{wermuth2011practice}; in scaffold hopping practice, arms (or fragments) are placed on the target surface first, then a scaffold (or linker) is placed to connect the arms \citep{schneider1999scaffold}. 
%\citep{imrie2020deep,huang20223dlinker,igashov2022equivariant}
Following the convention in traditional drug design, we aim to incorporate decomposed molecules, i.e., arms and scaffold, into deep generative models. 

% To tackle this problem, separating scaffolds and arms to decompose one large chemical space into the Cartesian product of several smaller chemical spaces is common in practical drug design. 
% In Figure~\ref{fig:decomp}, a ligand can be separated into a scaffold and arms. The arms are responsible for interacting with the receptor. The scaffold is responsible for positioning the arms into favorable interacting regions.
% This idea is also utilized in structure-based virtual screening \citep{sadybekov2022synthon}.
% need to show the idea in antibody design?
% However, the use of scaffold and arm decomposition is still under-explored in pocket-based 3D molecule generation.
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/decomp1.pdf}}
\caption{Ligand molecules can be decomposed into arms and scaffolds. 
Using MDM2 as an example, small molecule ligands are collected and displayed in the upper panel (colors represent different atom types). 
The ligand atoms are separated into arms and scaffolds based on their distance to the protein surface. 
Arms (lower right) form direct contact with the target, while scaffolds (lower left) connect the arms together.
Arm atoms are further clustered based on their positions, and the cluster (colored atom groups) show strong shape complementarity with local subpockets.}
\label{fig:decomp}
\vspace{-10mm}
\end{center}
\end{figure}

Recently, diffusion models have shown promise in many applications including SBDD, and offer suitable foundation for decomposable molecular generation. 
Before the prevalence of diffusion models, autoregressive models \citep{luo2021autoregressive,liu2022graphbp,peng2022pocket2mol} achieve the state-of-the-art (SOTA) performance in SBDD tasks, which generate 3D molecules in the target binding site by adding atoms and bonds iteratively. 
However, these models suffer from error accumulation and require a generation order, which is not trivial for molecular graphs.
% 3D molecule generation models show superiority to 2D-based models due to awareness of conformation which reflects some important properties of molecules, especially in the scenario of pocket-based molecule generation. 
%Autoregressive models, which hold strong expressive power in theory, are utilized to directly generate molecules in 3D space \citep{luo2021autoregressive,liu2022graphbp,peng2022pocket2mol}. 
%However, imposing a generation order on the molecular graph required by autoregressive models is non-trivial. Autoregressive models suffer from error accumulation and perform worse when generating larger molecules. 
Recent works \citep{anonymous2023de,schneuing2022structure,lin2022diffbp} leverage diffusion models \citep{ho2020denoising} to approximate the distribution of atom types and positions from a standard Gaussian prior, and use a post-processing algorithm to assign bonds between atoms. 
These methods can model local and global interactions between atoms simultaneously, and achieve better performance than autoregressive models.
Despite the SOTA performance, these methods have the following drawbacks 1) generating the entire ligand from a standard Gaussian prior can be inefficient as the 3D atom distribution is multimodal, 2) ignoring bonds in the modeling process can lead to unreasonable molecular structures.


In this paper, we propose \method, which is a new diffusion model with data-dependent decomposed priors for SBDD.
The decomposed priors respect the natural decomposition of a ligand when it interacts with a target. We also introduce a diffusion process on bonds to incorporate the bond generation in an end-to-end fashion instead of post-processing
To facilitate the generation process, we develop an additional validity guidance in the Langevin sampling, such as promoting the connection between the scaffold and arms and avoiding a geometric clash between the generated molecule and the target.
% Thus we propose a new diffusion model with data-dependent decomposed prior for pocked-based molecule generation, named DecompDiff, respecting the natural decomposition of a ligand when it interacts with a protein. 
% Besides, we introduce an additional drift term to guide the Langevin sampling towards our preferences, such as promoting the connection between the scaffold and arms and avoiding a geometric clash between the generated molecule and protein.

We highlight our main contributions as follows:
% \begin{itemize}
\begin{compactitem}
\item We propose a diffusion model with informative decomposed priors for structure-based drug design to incorporate the natural decomposition of a ligand molecule.
\item We introduce a bond diffusion procedure to simultaneously generate atoms and bonds for improving drug-likeness and synthesizability.
\item We design several guidance terms in the decomposed generation process to improve molecular validity. 
\item Our method can generate ligand molecules with better binding affinities measured by Vina and a higher success rate, achieving the new SOTA on the CrossDocked2020 benchmark.
\end{compactitem}




==> sections/31-related.tex <==
\section{Related Work}
\label{sec:related}


\paragraph{Molecule Generation}
Applying deep learning methods to molecule generation has shown promising results.
From the modalities of generated molecules, molecular generation research has gone through methods based on strings, graphs, and 3D structures.
In the initial stage, the string-based and graph-based methods dominate and achieve promising results in molecule generation.
The string-based methods~\citep{ kusner2017grammar,guimaraes2017objective,dai2018syntax,gomez2018automatic,flam2021keeping,eckmann2022limo,anonymous2023smilesformer,wang2022retrieval} represent the molecules with strings, such as SMILES~\cite{weininger1988smiles} and SELFIES~\cite{krenn2020self}, then regard the task as a sequence generation problem and borrow strong sequence generation models~(RNN, Transformer, etc.) used in natural language processing to solve such a string generation problem.
The graph-based methods~\citep{jin2018junction,jin2020hierarchical,liu2018constrained,de2018molgan,you2018graph,zang2020moflow,shi2020graphaf,luo2021graphdf,liu2021graphebm,bengio2021flow,ahn2021spanning,guo2022data,jo2022score,kong2022molecule,vignac2022digress,anonymous2023de,anonymous2023molebm,anonymous2023scorebased} regard atoms and bonds in the molecules as nodes and edges in the graph, respectively, and transform the molecular generation problem into a general graph generation problem.
However, such string-based and graph-based methods may unavoidably neglect some important geometric information of molecules in 3D spaces.

Hence, 3D-structure-based molecule generation methods have come. 
% \citep{gebauer2019symmetry,skalic2019shape,ragoza2020learning,simm2020reinforcement,ragoza2022generating,luo20213d,luo2021autoregressive,peng2022pocket2mol,schneuing2022structure,anonymous2023d} 

% Intuitively, although 1D strings and 2D graphs effectively simplify the molecular generation problem, considering that molecules live in 3D space, much important geometry information cannot be reasonably modeled and utilized in 1D strings and 2D graphs.

% Molecule Generation \citep{du2022molgensurvey} aims at generating molecules with desired properties that may facilitate downstream tasks such as drug discovery. Deep learning has shown promising results in molecule generation. In terms of modality, molecule generation can be categorized into 1D/2D-based and 3D-based. 

% 1D molecule generation methods leverage strings, such as SMILES \citep{weininger1988smiles} and SELFIES \citep{krenn2020self}, to represent molecules and formulate molecule generation as a sequence generation problem \citep{ kusner2017grammar,guimaraes2017objective,dai2018syntax,gomez2018automatic,flam2021keeping,eckmann2022limo,anonymous2023smilesformer,wang2022retrieval}. 
% 2D molecule generation methods view atoms as nodes and bonds as edges, and formulate molecule generation as a graph generation problem \cite{jin2018junction,jin2020hierarchical,liu2018constrained,de2018molgan,you2018graph,zang2020moflow,shi2020graphaf,luo2021graphdf,liu2021graphebm,bengio2021flow,ahn2021spanning,guo2022data,jo2022score,kong2022molecule,vignac2022digress,anonymous2023de,anonymous2023molebm,anonymous2023scorebased}. 

% However, in the physical world, molecules live in 3D space. Both 1D/2D molecule generation lacks such geometric information which acts as an important factor, especially in structure-based drug design. Thus recent mainstream pocket-based molecule generation methods directly generate molecules in 3D space \citep{gebauer2019symmetry,skalic2019shape,ragoza2020learning,simm2020reinforcement,ragoza2022generating,luo20213d,luo2021autoregressive,peng2022pocket2mol,schneuing2022structure,anonymous2023d}. 


\paragraph{Linker Design and Scaffold Elaboration}
In addition to \textit{de novo} design, there is another line of work on molecule design, which can be roughly divided into linker design and scaffold elaboration. 


\paragraph{Diffusion Models for Drug Design}
Diffusion models are emerging generative models that show promising results in generating images, text, and speech, and have also been introduced into drug design.

Diffusion models \citep{sohl2015deep,ho2020denoising,song2019generative} have shown promising results in image generation \citep{dhariwal2021diffusion,nichol2021glide,ramesh2022hierarchical}, text generation \citep{li2022diffusion}, and speech generation \citep{kong2021diffwave}. 
Diffusion models generate samples by iteratively denoising data points sampled from a standard Gaussian distribution. 
It can be extended to conditional or controllable generation via conditional input feature, classifier guidance \citep{dhariwal2021diffusion}, or classifier-free guidance \citep{ho2022classifier}. 
Besides, \citep{lee2021priorgrad} leverages conditional information as a non-standard Gaussian adaptive prior to further improve performance in speech synthesis. 
\cite{vignac2022digress} proposes a discrete model for graph generation and shows that the prior distribution closer to data distribution can induce superior performance.
